A cat qubit stabilization scheme using a voltage biased Josephson junction

DC-voltage-biased Josephson junctions have been recently employed in superconducting circuits for Hamiltonian engineering, demonstrating microwave amplification, single photon sources and entangled photon generation. Compared to more conventional approaches based on parametric pumps, this solution typically enables larger interaction strengths. In the context of quantum information, a two-to-one photon interaction can stabilize cat qubits, where bit-flip errors are exponentially suppressed, promising significant resource savings for quantum error correction. This work investigates how the DC bias approach to Hamiltonian engineering can benefit cat qubits. We find a simple circuit design that is predicted to showcase a two-to-one photon exchange rate larger than that of the parametric pump-based implementation while dynamically averaging typically resonant parasitic terms such as Kerr and cross Kerr. In addition to addressing qubit stabilization, we propose to use injection locking with a cat-qubit adapted frequency filter to prevent long-term drifts of the cat qubit angle associated to DC voltage noise. The whole scheme is simulated without rotating-wave approximations, highlighting for the first time the amplitude of related oscillatory effects in cat-qubit stabilization schemes. This study lays the groundwork for the experimental realization of such a circuit.

==> sections/results.tex <==
\section{Results}

\begin{itemize}
    \item Problem : DC assumed perfect previously, orders of magnitude et why it is problematic ( integrated noise worse than just noise )

    \item Implement Injection locking strategy in the context of cat qubits
( semi-classical ) mechanism explanation summary

    \item poser l'étude : 
e.o.m + classical simulations 

    \item results ( figure, phase space convergence, phase transition, arnold tingue ) 
\end{itemize}







